Integral representation of martingales motivated by the problem of endogenous completeness in financial economics

Let $\mathbb{Q}$ and $\mathbb{P}$ be equivalent probability measures and let $\psi$ be a $J$-dimensional vector of random variables such that $\frac{d\mathbb{Q}}{d\mathbb{P}}$ and $\psi$ are defined in terms of a weak solution $X$ to a $d$-dimensional stochastic differential equation. Motivated by the problem of \emph{endogenous completeness} in financial economics we present conditions which guarantee that every local martingale under $\mathbb{Q}$ is a stochastic integral with respect to the $J$-dimensional martingale $S_t \set \mathbb{E}^{\mathbb{Q}}[\psi|\mathcal{F}_t]$. While the drift $b=b(t,x)$ and the volatility $\sigma = \sigma(t,x)$ coefficients for $X$ need to have only minimal regularity properties with respect to $x$, they are assumed to be analytic functions with respect to $t$. We provide a counter-example showing that this $t$-analyticity assumption for $\sigma$ cannot be removed.

==> style.tex <==
% Packages
\RequirePackage[OT1]{fontenc}
\usepackage{amsthm} \usepackage{amsmath} \usepackage{amsfonts}
\usepackage{amssymb} \usepackage{latexsym} \usepackage{enumerate}
\usepackage[numbers]{natbib}
\usepackage{mathrsfs} \usepackage{enumitem}
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}

% Theorems and similar

\theoremstyle{plain}%
\newtheorem{Theorem}{Theorem}[section] %
\newtheorem{Corollary}[Theorem]{Corollary}%
\newtheorem{Lemma}[Theorem]{Lemma} %
\newtheorem{Proposition}[Theorem]{Proposition} %

\theoremstyle{definition}%
\newtheorem{Assumption}[Theorem]{Assumption}%
\newtheorem{Definition}[Theorem]{Definition}%
\newtheorem{Example}[Theorem]{Example} %
\newtheorem{Question}[Theorem]{Question}%
\newtheorem*{Acknowledgments}{Acknowledgments} %

\theoremstyle{remark}%
\newtheorem{Remark}[Theorem]{Remark} %


% Useful commands

\newcommand{\abs}[1]{\lvert#1\rvert} % absolute value
\newcommand{\braces}[1]{\lbrace{#1}\rbrace} % braces around
\newcommand{\descr}[2]{\lbrace{#1}:\; #2 \rbrace} % description
\newcommand{\im}{{i}} % imaginary i
\newcommand{\ind}[1]{1_{\{#1\}}}
\newcommand{\ip}[2]{{#1}{#2}} % scalar product
\newcommand{\map}[3]{#1:\; #2 \rightarrow #3} %1=name, 2=arg_domain, 3=val_domain
\newcommand{\mtext}[1]{\;\text{#1}\;} % text in the middle of a formula
\newcommand{\norm}[1]{\lVert#1\rVert} %
\newcommand{\set}{\triangleq} % definition of  something
\newcommand{\setind}[1]{1_{#1}}

% Mathematical operators

\DeclareMathOperator{\esssup}{ess\,sup} 
\DeclareMathOperator{\trace}{trace}


% Numbering

\numberwithin{equation}{section}

% Counters

\newcounter{item} 
